VCD: A Dataset for Visual Commonsense Discovery in Images

Visual commonsense plays a vital role in understanding and reasoning about the visual world. While commonsense knowledge bases like ConceptNet provide structured collections of general facts, they lack visually grounded representations. Scene graph datasets like Visual Genome, though rich in object-level descriptions, primarily focus on directly observable information and lack systematic categorization of commonsense knowledge. We present Visual Commonsense Dataset (VCD), a large-scale dataset containing over 100,000 images and 14 million object-commonsense pairs that bridges this gap. VCD introduces a novel three-level taxonomy for visual commonsense, integrating both Seen (directly observable) and Unseen (inferrable) commonsense across Property, Action, and Space aspects. Each commonsense is represented as a triple where the head entity is grounded to object bounding boxes in images, enabling scene-dependent and object-specific visual commonsense representation. To demonstrate VCD's utility, we develop VCM, a generative model that combines a vision-language model with instruction tuning to discover diverse visual commonsense from images. Extensive evaluations demonstrate both the high quality of VCD and its value as a resource for advancing visually grounded commonsense understanding and reasoning. Our dataset and code will be released on https://github.com/NUSTM/VCD.

==> secs/5_evaluation_on_main.tex <==
% \section{Evaluation of \model{} on \task{}}
% This section describes the experimental setup and presents the performance of \model{} on \task{}.
% We also provide the evaluation of \model{} on downstream tasks in App.~\ref{sec:evaluation_of_downstream_tasks}.

% \subsection{Evaluation Protocol}

% \paragraph{Automatic Evaluation Metrics}
% For the automatic evaluation of \model{}'s visual commonsense discovery capabilities, we employ metrics for natural language generation: BLEU-1 (B-1)~\citep{bleu}, BLEU-2 (B-2), Rouge-L (R)~\citep{rouge}, METEOR (M)~\citep{meteor}, and Word Error Rate (W)~\citep{wer}.

% \paragraph{Human Evaluation Metrics}

% While automatic evaluation metrics provide preliminary insights, they may not fully capture the diversity and quality perceived by humans.
% Therefore, we conduct a human evaluation, focusing on the correctness and completeness of commonsense generated by \model{}.
% For each type of visual commonsense, 10 images are randomly selected.
% Their associated outputs are compared against those produced by multimodal large language models (MLLMs).
% Two independent evaluators analyze the results, and any disagreements are resolved by a third.
% The evaluations are structured as win/draw/lose comparisons.
% Evaluators receive salary at a rate of \$8 per hour, which is above the local average wage.

% \subsection{Main Results}

% Based on OFA standard architecture, we evaluate the performance of \model{} across various scales.
% Detailed model configurations are provided in App.~\ref{sec:model_config}.
% % MLLMs, \eg, Shikra~\citep{shikra} and SPHINX~\citep{sphinx}, might outperform OFA as backbones but are not used due to high computational costs.
% % However, the massive parameters of MLLMs demand computational resources beyond our capability.
% % These models exhibit substantial zero-shot learning abilities by harnessing power of large language models.
% We select the highe-ranking open and closed source MLLMs on MME leaderboard~\cite{mme}, SPHINX and GPT-4V~\cite{gpt4}, and then manually compare them with \model{}$_{\text{large}}$ by carefully crafting the prompts.
% The crafted prompts and qualitative results are illustrated in App.~\ref{sec:prompts} and App.~\ref{sec:qualitative}.

% \subsubsection{Automatic Evaluation}

% Tab.~\ref{table:main_results} summarizes the results of the automatic evaluation.
% Upon analyzing the results in Tab.~\ref{table:main_results}, we can find that
% \model{} exhibits improvements in all automatic evaluation metrics as the model scale increases, which is consistent with our expectations.
% Particularly, \model{}$_{\text{tiny}}$ shows a significant decrease in performance, highlighting the importance of the model scale for \task{}.

% \input{tables/main_results}

% \input{tables/human_evaluation}

% \subsubsection{Human Evaluation}

% Human evaluation results are summarized in Tab.~\ref{table:human_evaluation}.
% \model{}${\text{large}}$ outperforms \model{}${\text{base}}$ in both explicit and implicit commonsense tasks, aligning with automatic evaluation results and affirming the reliability of automatic metrics.
% It also significantly outperforms SPHINX, which struggles with instruction adherence, particularly in identifying implicit commonsense.

% GPT-4V excels in \task{}, effectively generating diverse explicit and implicit commonsense as instructed.
% Notably, it surpasses \model{}${\text{large}}$ in explicit commonsense discovery, producing more varied examples.
% However, GPT-4V underperforms in implicit commonsense discovery, often mixing explicit and implicit concepts.
% This suggests it understands the distinction but fails to generate them distinctly.
% In contrast, \model{}${\text{large}}$ better associates implicit commonsense with image elements.

% Fleiss’ kappa scores indicate moderate agreement among annotators, demonstrating reliable evaluation.

% \subsection{Ablation Study}

% To evaluate the impact of images, bounding boxes, and object names on \model{}’s performance, we conduct ablation studies.
% Results in Tab.~\ref{table:main_results} show that removing any of these elements degrades performance, with the removal of object names causing the most significant drop, even below \model{}$_\text{base}$.
% This highlights the critical role of textual information from object names.

% Interestingly, \model{}$_\text{large}$ performs better without images than with images lacking bounding boxes.
% This suggests that bounding boxes are essential for guiding visual commonsense discovery, as their absence introduces ambiguity about the target object in complex scenes.
% Additionally, the presence of multiple objects with identical names can further hinder visual commonsense discovery.

==> tables/comparison_year.tex <==
\begin{table*}[t]
\center
\caption{Comparison with other datasets related to visual commonsense.}
\begin{adjustbox}{max width=1.\linewidth}
\begin{tabular}{@{}lccccc@{}}
\toprule
                            & Explicit & Implicit & \# Categories & \# Images & \# Commonsense \\ \midrule
ConceptNet (2017)             &    \ding{52}      &   \ding{52}       & 34            &    \ding{56}       & $\approx$400M           \\
Visual Genome (2017)          &    \ding{52}      &      \ding{56}    & \ding{56}             &    $\approx$106K       &       $\approx$5M         \\
SpatialCS (2022)   &          \ding{52}        &   \ding{56}          & 1             & \ding{56}          & 1224           \\
ViComTe (2022)               &          \ding{52}        &   \ding{56}          & 6             & \ding{56}         & 11114          \\
VEC (2023) &          \ding{52}        &   \ding{56}          & 8             & \ding{56}          & 4090           \\
% ROME~\citep{rome}                &          \ding{52}        &   \ding{56}          & 5             & 1563      & \ding{56}             \\ 
VIPHY (2023)                 &   \ding{52}        &   \ding{56}        & 3             & \ding{56}          & $\approx$30K            \\
ImageNetVC (2023)             &          \ding{52}        &   \ding{56}          & 6             & \ding{56}         & 4976           \\
\midrule
VKB                    &          \ding{52}        &   \ding{52}          & 11            &      $\approx$106K     &       $\approx$7M       \\ \bottomrule
\end{tabular}
\end{adjustbox}
\label{table:comparison}
\end{table*}

==> tables/vcs.tex <==
\begin{table}[t]
\center
\caption{Types of visual commonsense in the hierarchical form.}
\begin{adjustbox}{max width=1.\columnwidth}
\begin{tabular}{@{}llc@{}}
\toprule
\multirow{3}{*}{Explicit} & Property                & \textit{/E/P/HasProperty}                    \\ \cmidrule(l){2-3} 
                          & Space                 & \textit{/E/S/LocatedNear, /E/S/Relatedness}  \\ \cmidrule(l){2-3} 
                          & Action                  & \textit{/E/A/CapableOf, /E/A/ReceivesAction} \\ \midrule
\multirow{4}{*}{Implicit} & Property                & \textit{/I/P/HasProperty, /I/P/CreatedBy}    \\ \cmidrule(l){2-3} 
                          & Space                 & \textit{/I/S/LocatedNear}                    \\ \cmidrule(l){2-3} 
                          & \multirow{2}{*}{Action} & \textit{/I/A/CapableOf, /I/A/UsedFor,}       \\
                          &                         & \textit{/I/A/ReceivesAction}                 \\ \bottomrule
\end{tabular}
\end{adjustbox}
\label{table:category}
\end{table}
